k-Convex Polyominoes by Semi-perimeter

We give the conjectured solution for the generating function of k-convex polyominoes, enumerated by semi-perimeter. The solution was obtained from the analysis of enumeration data that we generated.

==> eptcsdata.tex <==
\providecommand{\firstpage}{74}
\providecommand{\publicationstatus}{S. Brlek and L. Ferrari (Eds.): GASCom 2026\\
EPTCS 445, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.445.10}{10.4204/EPTCS.445.10}}
\pdfoutput=1

